Predicting Choice with Set-Dependent Aggregation

Providing users with alternatives to choose from is an essential component in many online platforms, making the accurate prediction of choice vital to their success. A renewed interest in learning choice models has led to significant progress in modeling power, but most current methods are either limited in the types of choice behavior they capture, cannot be applied to large-scale data, or both. Here we propose a learning framework for predicting choice that is accurate, versatile, theoretically grounded, and scales well. Our key modeling point is that to account for how humans choose, predictive models must capture certain set-related invariances. Building on recent results in economics, we derive a class of models that can express any behavioral choice pattern, enjoy favorable sample complexity guarantees, and can be efficiently trained end-to-end. Experiments on three large choice datasets demonstrate the utility of our approach.

==> ablation_details_table.tex <==
% !TEX root = choice_nips19.tex

% Table generated by Excel2LaTeX from sheet 'results-ablation'




==> agg_table.tex <==
% !TEX root = choice_nips19.tex

\begin{table*}[!htb]
	\centering
	  \fontsize{8pt}{9.5pt}\selectfont
		\caption{\todo{Add caption}}
% Table generated by Excel2LaTeX from sheet 'table2'
\begin{tabular}{cllll}
	Type & Extends & $w$ & $r$ & $\mu$ \\
	\toprule
	- & \cite{mcfadden1973conditional} & one & zero & identity \\
	\midrule
	\multirow{4}[2]{*}{I} & \cite{tversky1969intransitivity} & (max-min)$^\rho$ & zero & identity \\
	& \cite{mcfadden1978modeling} & linear & log $\sum$ exp & log \\
	& \cite{kalai2002rationalizing} & softmax & zero & identity \\
	& \cite{orhun2009optimal} & linear & w. average & kinked lin. \\
	\midrule
	\multirow{3}[2]{*}{II} & \cite{kaneko1979nash} & sum & min & log \\
	& \cite{kivetz2004alternative} (LAM) & sum & (max+min)/2 & kinked lin. \\
	& \cite{kivetz2004alternative} (CCM) & sum & min & power$(\rho)$ \\
	\midrule
	\multirow{2}[2]{*}{III} & \cite{kivetz2004alternative} (NCCM) & max-min & min & norm. pow$(\rho)$ \\
	& Ours & set-nn & set-nn & kinked tanh \\
	\bottomrule
\end{tabular}%
	\label{tbl:table_agg}%
\end{table*}


==> model.tex <==
% !TEX root = choice_nips19.tex

\section{Model Specification} \label{sec:model_specs}

Thus far we have considered only general forms of aggregation.
We now proceed to presenting a specific aggregation model
which is well-suited for choice prediction.
Our model strikes a balance between flexibility (by satisfying certain invariances)
and specificity (using appropriate inductive bias).

We propose the following form of aggregation:
\beq
g(x,s) = \big\langle w(s), \nonlin_d \big( \f(x), \r(s) \big) \big\rangle.
\label{eq:agg}
\eeq
We now elaborate on the different components of $\agg$.
For a single dimension $i \in [\ell]$ in the embedded space,
items are first evaluated using some $f_i(x) \in \F$.
Then, a ``reference'' valuation is constructed
via a set function $r_i(s)$.
Next, $f_i(x)$ and $r_i(s)$ are compared by a scalar operator $d(\cdotp,\cdotp)$,
such as $d(a,b)=a-b$. % for scalar values or $d(a,b)=\inner{a,b}$ for vectors.
We have found it useful to generalize this by letting $f_i$ and $r_i$ be vector valued,
and setting $d$ to be an inner product.
The item-reference relation is then fed into an a-symmetric non-linearity $\nonlin(\cdotp)$.
We denote by $\mu_d$ the composition of $\mu$ over $d$.
Finally, all $\ell$ valuations are aggregated using set-dependent weights $w(s)$.
Figure \ref{fig:diagram} presents a diagram of this setup.

Eq. \eqref{eq:agg} injects inductive bias 
inspired by the following key principles in behavioral choice theory:
\begin{enumerate}[label=\textbf{P\arabic*}:,ref=P\arabic*]
%\begin{enumerate}[leftmargin=1.5em]
	\setlength\itemsep{0.2em}
	
	\item \label{p:nonlin}
	\textbf{Asymmetry.} 
	Losses and gains are perceived in an a-symmetric, non-linear manner.
	This is the hallmark of Kahneman and Tversky's Prospect Theory
	\cite{kahneman1979prospect,tversky1992advances}.
	
	\item \label{p:r}
	\textbf{Relativity.}
	Valuations are relative, and are considered with
	respect to a mutual (and possibly hypothetical) referral item \cite[e.g., ][]{tversky1991loss}.
	
	\item \label{p:w}
	\textbf{Integrability.}	
	Subjective value is multi-dimensional,
	and context determines how valuations are integrated into a single choice
	\cite[e.g., ][]{tversky1969intransitivity, tversky1993context}.
%\end{enumerate}
\end{enumerate}
%These serve as appropriate inductive bias for predicting on real choice data.

\begin{proposition}
	$g(x,s)$ in Eq. \eqref{eq:agg} satisfies  \ref{p:nonlin},
	\ref{p:r}, and \ref{p:w}.
\end{proposition}
To see this, note that for each dimension $i$,
item scores $f_i(x)$ are compared to a mutual set-dependent reference point $r_i(s)$
via $d$, satisfying \ref{p:r}.
Using a pointwise a-symmetric non-linearity for $\nonlin$ gives \ref{p:nonlin}.
Finally, in accordance with \ref{p:w}, valuations are aggregated
in $\agg$ via $\w(s)$. 

We now describe our specific choice of components.
We model $w(s)$ and $r(s)$ as set neural networks \cite{zaheer2017deep}.
These are general neural networks whose architecture guarantees permutation
invariance, meaning that permuting $s$ will not change the output.
For the scalar function $\nonlin$, we have found it useful to use a kinked tanh function:
\[
\nonlin(z) =  c \tanh(z) \cdotp \one{z<0} + \tanh(z) \cdotp \one{z\ge0}, \quad c>1
\]
which is inspired by the s-shaped utility functions used in prospect theory \cite{maggi2004characterization}.

Since all four elements of $\agg$ are differentiable,
$\agg$ can be optimized over any appropriate loss function (i.e., cross entropy)
using standard gradient methods.
The learned parameters include the weights in $w$ and in $r$,
and $c$ for $\nonlin$.
We note that Eq. \eqref{eq:agg} encompasses several models from the multi-self literature.
Since these are usually designed for mathematical tractability,
they do not always include explicit functional forms,
and use simple non-parametric set operations for $w$ and $r$.
The predictive advantage of our parametrized model is demonstrated empirically
in Sec. \ref{sec:agg_vs_ms}.


\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=0.3\columnwidth]{diagram3}
		\caption{The proposed aggregation model}
		\label{fig:diagram}
	\end{center}
\end{figure}




\input{results_table}




%\red{======================}
%
%\subsection{Inductive bias}
%In Sec. \ref{sec:model} we argure that violating IIA is possible
%only if choice is modeled using set functions.
%General set functions, however,
%have not guarantees regarding violation expressivity,
%and are unlikely to capture behavioral violations found in real choice data.
%We therefore turn to the literature on behavioral choice,
%and identify three key principles:
%%We construct our model to directly encode key principles from behavioral choice theory.
%%A large and growing body of evidence suggests that people violate IIA regularly and in consistent manners \cite{simonson1989choice, simonson1992choice, busemeyer1993decision, tversky1993context, wernerfelt1995rational, sedikides1999contextual, benartzi2002much, latty2010irrational, berkowitsch2014rigorously, neumann2016meta},
%%and several choice models have been proposed to capture these effects
%%\cite{tversky1972elimination, kivetz2004alternative, orhun2009optimal, rooderkerk2011incorporating}.
%%Three recurrent principles can be extracted from the above:
%\begin{enumerate}[label=\textbf{P\arabic*}:,ref=P\arabic*]
%	\item \label{p:nonlin}
%	\textbf{Asymmetry.} 
%	Losses and gains are perceived in an a-symmetric, non-linear manner.
%	This is the hallmark of Kahneman and Tversky's renowned Prospect Theory
%	\cite{kahneman1979prospect,tversky1992advances}.
%	
%	\item \label{p:r}
%	\textbf{Relativity.}
%	Item valuations are relative, and are considered with
%	respect to a mutual (and possibly hypothetical) referral item \cite[e.g., ][]{tversky1991loss}.
%	
%	\item \label{p:w}
%	\textbf{Integrability.}	
%	Subjective value is multi-dimensional,
%	and context determines how valuations are integrated into a single choice
%	\cite[e.g., ][]{tversky1969intransitivity, tversky1993context}.
%\end{enumerate}
%\todo{add citations}
%
%In line with these, 
%%which we encode into our general aggregation model  in Eq. \ref{eq:agg_typeIII}.
%we propose to instantiate $\agg(x,s)$ in Eq. \ref{eq:agg_typeIII} in the following way.
%For a single dimension $i \in [\ell]$ in the embedded space,
%items are first evaluated using some $f_i(x) \in \F$.
%Then, a ``reference'' valuation is constructed
%via a set function $r_i(s) = r(f_i(s))$,
%where $f_i(s) = (f_i(x_1),\dots,f_i(x_n))$.
%Next, $f_i(x)$ and $r_i(s)$ are compared by a scalar operator $d(\cdotp,\cdotp)$,
%such as $d(a,b)=a-b$. % for scalar values or $d(a,b)=\inner{a,b}$ for vectors.
%The item-reference relation is then fed into an a-symmetric non-linearity $\nonlin(\cdotp)$.
%We denote by $\mu_d$ the composition of $\mu$ over $d$.
%Finally, all $\ell$ valuations are aggregated using set-dependent weights $w(s)$
%with $w_i(s)=w(f_i(s))$, giving the aggregator:
%\beq
%g(x,s) = \big\langle w(s), \nonlin_d \big( \f(x), \r(s) \big) \big\rangle.
%\label{eq:agg}
%\eeq
%
%
%
%\begin{proposition}
%	The aggregator $g(x,s)$ in Eq. \eqref{eq:agg} satisfies  \ref{p:nonlin},
%	\ref{p:r}, and \ref{p:w}.
%\end{proposition}
%To see this, note that for each dimension $i$,
%item scores $f_i(x)$ are compared to a mutual set-dependent reference point $r_i(s)$
%via $d$, satisfying \ref{p:r}.
%Using a pointwise a-symmetric non-linearity for $\nonlin$ gives \ref{p:nonlin}.
%Finally, in accordance with \ref{p:w}, valuations are aggregated
%in $\agg$ via $\w(s)$. 
%
%We now present our choice of components for Eq. \eqref{eq:agg}.
%
%\todo{we use multi-variate $u$}
%
%\subsection{Invariance}
%\blue{
%As we \blue{show in the Appendix},
%Eq. \eqref{eq:agg} generalizes several models from the multi-self literature.
%However, since their main focus is in most cases on mathematical tractability,
%their choices for $r,w,d$, and $\nonlin$ are restricted to simple operators.
%%such as demonstrating contextual effects \cite{kivetz2004alternative}
%%or proving impossibility results \cite{kalai2002rationalizing}.
%As our goal is to promote predictive accuracy,
%rather than choose specific functional forms,
%we restrict the components in terms of the invariances they must preserve.
%
%As we argue in Sec. \ref{sec:pred_choice}, violations can arise only 
%if the model is defined using set functions.
%This means that $\agg$ must be permutation invariant:
%For any permutation
%of items $\pi: [n] \rightarrow [n]$, it must hold that
%$\agg(x,s) = \agg(\pi(x),\pi(s))$. %,
%%where $\agg(s) = (\agg(x_1,s),\dots,\agg(x_n,s))$ and $\pi$ is applied element-wise.
%A recent result by \cite{zaheer2017deep}
%shows that using certain compositional rules,
%to guarantee that $\agg$ is permutation equivariant,
%it suffices to guarantee that each $w_i$ and $r_i$ %(which are scalar functions)
%are permutation invariant, meaning that $w_i(s) = w_i(\pi(s))$, and likewise $r_i$.
%We follow \cite{zaheer2017deep}
%and model the components of $\agg$ using appropriate general-purpose neural networks.
%For $\w$ and $\r$, we use the permutation invariant neural networks 
%with max pooling. % as suggested in \cite{zaheer2017deep}.
%For the scalar function $\nonlin$, we have found it useful to use a kinked tanh function:
%\[
%\nonlin(z) =  c \tanh(z) \cdotp \one{z<0} + \tanh(z) \cdotp \one{z\ge0}, \quad c>1
%\]
%which is inspired by the s-shaped utility functions used in prospect theory \cite{maggi2004characterization}.
%Finally, $f_i$ can be chosen according to the nature of the data. In our case,
%we use fully connected neural networks with tanh activations.
%Figure \ref{fig:diagram} presents a diagram of our final aggregation model.
%
%Since all four elements of $\agg$ are differentiable,
%$\agg$ can be optimized over any appropriate loss function (i.e., multinomial logistic loss)
%using standard gradient methods.
%
%\todo{explicitly state the learned parameters}
%
%- parametric set funcs
%- multi-var f
%}


%\red{=======================================}
%
%\blue{
%Given data on alternatives and choices,
%one natural approach is to cast choice prediction as ranking problem.
%This typically involves learning an item score (or ``utility'') function $f(x)$ over items,
%such that within each given set, the chosen item is scored higher than all non-chosen items.
%Each choice instance is hence teated as an observed partial ranking.
%In a discriminative approach, $f$ is chosen from some class $F$
%to minimize an appropriate loss.
%Prediction over a set is then made by taking the highest-scoring item, namely:
%\beq
%\label{eq:argmax_f}
%h(s) = \argmax_{x \in s} f(x)
%\eeq
%
%\blue{There are many variations on this idea \toref.}
%However, any approach based on Eq. \eqref{eq:argmax_f}
%\blue{is predestined to follow IIA,} \todo{verify this}
%regardless of the complexity or expressive power of $f$.
%Trivially, this is because the highest-scoring item in a set
%will not change if lower-scoring items are removed. \todo{redundant? also mentioned in intro}
%
%This implies that, in order to allow for violations of IIA,
%the score function should take into account not only $x$,
%but also all other items in $s$.
%We therefore propose to replace the item function $f(x)$ in Eq. \eqref{eq:argmax_f}
%with a \emph{set function} $\agg(x;s)$,
%where the score of each $x \in s$ depends on $s$.
%The prediction rule becomes:
%\beq
%\label{eq:argmax_g}
%h(s) = \argmax_{x \in s} \agg(x;s)
%\eeq
%The main difference in Eq. \eqref{eq:argmax_g} is that now, since $\agg$ depends on $s$,
%the same item can be scored differently when contained in different sets.
%This means that predictions can potentially change when items are removed from $s$,
%which is a necessary condition for allowing IIA violations.
%
%While it is possible to model $\agg$ as a general set function,
%this does not provide any guarantees on what violations it can express.
%In what follows, we elaborate on the properties that $\agg$ 
%should hold in order to support arbitrary IIA violations,
%and present a rich class of appropriate functions that are well suited for choice prediction.
%
%
%
%\subsection{Violation by aggregation}
%
%%\todo{stress the point that on one hand we'd like models that are as general as possible (under the required invariances), and on the other hand that we'd like to imbue powerful prior knowledge in the models to serve as inductive bias}
%
%One way to deviate from IIA
%is to aggregate multiple item functions in a context-dependent manner.
%\blue{
%	Consider, for example, a diner at a restaurant who wishes to order wine.
%	Looking at the wine menu, the diner finds out that wine is frustratingly more expensive than
%	she had thought.
%	Nonetheless, she would still like to have wine.
%	On the one hand, she does not want to spend too much;
%	on the other hand, she does not want to appear cheap.
%	Looking at the menu again, she decides to order the second cheapest wine.
%	%The ``second cheapest wine'' phenomena, and others like it, are widespread
%	%and extremely common in everyday choice.
%	The key insight here is that choice depends 
%	not only on intrinsic item properties (e.g., price),
%	but also on an item's relation to the set of alternatives (e.g., the item's price rank).
%}
%\todo{ref kalai 2002, sen 1993 (see AR)}
%
%\blue{
%	Formally, $\agg$ is modeled to combine a collection of $\ell$ item functions
%	$\f = (f_1,\dots,f_\ell)$ in a way that depends on $s$.
%	%which we write as $\agg(\f(x);s)$. %$\agg\left(\{f_i(x)\}_{i=1}^\ell;s\right)$. %$\agg(f_{1:\ell}(x);s)$
%	This idea is fundamental to Arrow's impossibility result in social choice \cite{arrow1951social},
%	which has motivated a rich literature in choice theory based on models of multiple ``selves''
%	(where each $f_i$ is thought of as a rational ``self'').
%}
%From the seminal work of \cite{may1954intransitivity}, mutli-self models have been studied in
%economics \cite{kalai2002rationalizing, fudenberg2006dual, manzini2007sequentially, green2007choice, liang2015interpretation},
%marketing \cite{kivetz2004alternative, orhun2009optimal} %, rooderkerk2011incorporating},
%and psychology \cite{tversky1969intransitivity, shafir1993reason, tversky1993context}.
%\todo{add papers of example models from AR}
%%\tocitec{Tversky (1969), Shafir, Simonson and Tversky (1993) and Tversky and Simonson (1993)}.
%%\green{Since the seminal work of May (1954), formal
%%models of multi-self decision-making proposed include Kalai, Rubinstein and Spiegler (2002),
%%Fudenberg and Levine (2006), Manzini and Mariotti (2007), and Green and Hojman (2009)
%%in the economics literature, where selves are often seen as rationales or manifestations of
%%temptation and self control processes; Kivetz, Netzer and Srinivasan (2004) in the marketing
%%literature, where selves are different considerations or criteria for evaluating products; and
%%Tversky (1969), Shafir, Simonson and Tversky (1993) and Tversky and Simonson (1993) in
%%the psychology literature, where the multiplicity of self, comprised of different motivational
%%systems, has long been viewed as a normal feature instead of a sign of pathology. [AR]}
%
%\todo{revisit wine example}
%
%Models such as the above are typically designed with a specific goal in mind,
%such as portraying a certain type of behavioral tendency
%or satisfy a set of axioms.
%More often than not, this comes at the price of generality and predictive power.
%However, reviewing the literature provides insight into three recurrent principles:
%\begin{enumerate}[label=\textbf{P\arabic*}:,ref=P\arabic*]
%	\item \label{p:nonlin}
%	Losses and gains are perceived in an a-symmetric, non-linear manner;
%	%Value is a-symmetric in terms of losses versus gains, and typically non-linear;
%	this is the hallmark of Kahneman and Tversky's renowned Prospect Theory \tocite.
%	
%	\item \label{p:r}
%	Item valuations are relative, and are often with
%	respect to a mutual (and possibly hypothetical) referral item.
%	
%	\green{Amos Tversky and Daniel Kahneman’s
%		(1991) theory of reference-dependent preferences, in which an individual’s preferences over
%		bundles of goods are conditional on his or her reference point
%		[The Imbalanced Luce Model,
%		On the theory of reference-dependent preferences]
%	}
%	
%	\item \label{p:w}
%	Subjective value is multi-dimensional, and context affects how different
%	valuations form into a single choice.
%\end{enumerate}
%
%\subsection{Proposed aggregation model}
%
%
%%\begin{figure}[t]
%%	\begin{center}
%%		\includegraphics[width=0.75\columnwidth]{diagram2}
%%		\caption{\todo{...}}
%%		\label{fig:diagram}
%%	\end{center}
%%\end{figure}
%
%
%\todo{REDO THIS SECTION}
%
%Treating the above principles as guidelines for inductive bias,
%we propose the following general form of utility aggregation:
%\beq
%\label{eq:agg}
%\agg(x;s) = \sum_{i=1}^\ell w_i(s) \cdotp \nonlin \big( f_i(x)-r_i(s) \big)
%\eeq
%or more compactly in vector notation:
%\beq
%\label{eq:agg_vec}
%g(x;s) = \inner{\w(s), \feat(x;s)}, \quad \feat(x;s) = \nonlin (\f(x)-\r(s)) %\nonumber
%\eeq
%where $\nonlin:\R \rightarrow \R$ and $\w, \r : 2^\X \rightarrow \R^\ell$. 
%The various components of $\agg$ implement the ideas presented above.
%In line with \ref{p:w}, the item functions $f_i$ play the role of different
%valuation mechanism. As a vector, $\feat(x)$ represents
%the item $x$ in some latent $\ell$-dimensional utility space.
%Following \ref{p:r}, item scores $\f(x)$ are compared to a mutual
%set-dependent reference point $\r(s)$.
%Then, using \ref{p:nonlin}, 
%a pointwise a-symmetric non-linearity $\nonlin$ is applied,
%giving a set-specific item representation $\feat(x;s)$.
%Finally, going back to \ref{p:w}, utilities are aggregated
%via a weighted sum using set-dependent weights $\w(s)$.
%
%\todo{replace selves with embedding dimension when appropriate} \\
%\todo{stress that just $f$ or aggregating without set dependence cannot break IIA by definition}
%
%Eq. \eqref{eq:agg_vec} provides an interesting interpretation of $\agg$.
%Conditional on $s$, $g$ is a simple linear \blue{ranker/classifier/score functions} applied to
%some feature representation of $x$ (in this case, $\feat$).
%However, for different sets, both weights \emph{and} feature representation may change.
%\blue{When both $\feat$ and $\w$ are parametrized, this means that both feature representations and weights are learned.}
%%From the perspective of IIA,
%When an item $x$ is removed from a set $s$,
%the remaining points move and the hyperplane rotates.
%This makes it possible to have $h(s) \neq h(s \setminus \{x\})$ (see Eq. \eqref{eq:iia_rmv1}),
%and is the manner in which $\agg$ allows for IIA violations.
%Figure \ref{fig:viol_viz} illustrates this idea using a real example from our experiments.
%
%\todo{agg class $\Agg$ induced by base class $F$}\\
%\todo{build up for general diff. aggs}
%
%
%
%
%%\todo{make it clear that this is our contribution}
%
%
%\subsection{\blue{Working with universal aggregators}}
%The form of $\agg$ in Eq. \eqref{eq:agg} generalizes
%many of the multi-selves models mentioned earlier,
%which account for certain instantiations of $\w,\r$, and $\nonlin$
%(see Table \toref).\footnote{
%	In most models, $\w$ and $\r$ decompose over selves and explicitly operate on $f(x)$.
%	For generality, we have opted to express them as vector functions of $s$.}
%\todo{add model table}
%As noted above, these may not be ideal for predictive purposes.
%Following \tocitec{deep sets}, we propose to model $\w$ and $\r$
%as general vector-valued set functions (i.e., with appropriate neural networks),
%and $\nonlin$ as a parametric non-linearity. \todo{elaborate more on $\nonlin$ - loss aversion, etc}
%As a set function, $\agg$ is required to preserve permutation equivariance,
%meaning that permuting the items should also permute item scores in the same manner.
%The linearity of aggregation guarantees that this holds as long
%as $\w$ and $\r$ are element-wise permutation invariant \tocitec{deep sets?}.
%When all four elements of $\agg$ are differentiable,
%$\agg$ can be optimized over any appropriate loss function (i.e., multinomial logistic loss)
%using standard gradient methods.
%
%
%\todo{clarify the novelty of this idea}\\ 
%\todo{AR? violation counts?}
%
%
%The functional form of $\agg$ makes it possible to express violations of IIA.
%This, however, does not provide any notion of what \emph{which} violations it can express.
%Rather than targeting specific types,
%we aim to allow for arbitrary violations,
%so that learning can capture any violations that may exist in the data.
%In the next section, we show that
%$\agg$ can potentially express any violation,
%and is limited only by the expressivity of the base class $F$
%and the representation dimension $\ell$.
%}
